The effect of ambient air pollution on birth outcomes in Norway

Ambient air pollution is harmful to the fetus even in countries with relatively low levels of pollution. In this paper, I examine the effects of ambient air pollution on birth outcomes in Norway. I find that prenatal exposure to ambient nitric oxide in the last trimester causes significant birth weight and birth length loss under the same sub-postcode fixed effects and calendar month fixed effects, whereas other ambient air pollutants such as nitrogen dioxide and sulfur dioxide appear to be at safe levels for the fetus in Norway. In addition, the marginal adverse effect of ambient nitric oxide is larger for newborns with disadvantaged parents. Both average concentrations of nitric oxide and occasional high concentration events can adversely affect birth outcomes. The contributions of my work include: first, my finding that prenatal exposure to environmental nitric oxide has an adverse effect on birth outcomes fills a long-standing knowledge gap. Second, with the large sample size and geographic division of sub-postal codes in Norway, I can control for a rich set of spatio-temporal fixed effects to overcome most of the endogeneity problems caused by the choice of residential area and date of delivery. In addition, I study ambient air pollution in a low-pollution setting, which provides new evidence on the health effects of low ambient air pollution.

==> tables/des_i_p.tex <==
\begin{table}[htbp]
\centering
\caption{Infantile and parental information \label{tab:balance_i_p}}

\begin{threeparttable}
\begin{tabular}{l*{6}{c}}
\toprule
 Variable   &     mean&  s.d.&  min & max  &  obs.(1000) \\
\midrule

\multicolumn{2}{l}{A. Infantile Information} \\

$weight(g)$      &     3507.34&      600.66&    0&     7,070&     1,008  \\
$length(cm)$      &       50.05&        2.70&     0&       99&      972  \\
$gender$      &        0.51&        0.50&        0&        1&     1,009  \\
\midrule

\multicolumn{2}{l}{B. Time} \\

$year$       &     2008.10&        4.87&     2000&     2016&      1,009  \\
$month$       &      582.57&       58.60&      480&      683&     1,009  \\
\midrule

\multicolumn{2}{l}{C. Parental Information} \\

$age_m$       &       30.31&         5.14&        13&         60&      980  \\
$edu_m$       &        5.00&         1.53&         0&          8&      966   \\
$edu_f$       &        4.71&         1.53&         0&          8&      952  \\
$native_m$    &        0.89&         0.31&         0&          1&    1,004 \\
$native_f$    &        0.90&         0.30&         0&          1&      983  \\
$img_m$      &         0.75&         0.43&         0&          1&    1,004 \\
$img_f$      &         0.77&         0.42&         0&          1&      983  \\
$income_m$    &      209.35&       252.49&   -15,302&    141,432&      952  \\
$income_f$    &      294.27&       744.16&  -194,175&    330,406&      947  \\
$wealth_m$    &      315.77&     2,545.89&      -801&  1,039,671&      952  \\
$wealth_f$    &      460.22&     2,796.02&         0&  1,102,742&      947  \\
$debt_m$      &      430.56&       792.67&         0&    175,208&      952  \\
$debt_f$      &      928.13&     1,753.48&         0&    835,383&      947  \\
\bottomrule

\end{tabular}

\begin{tablenotes}
      \small
      \item Notes: (1)Subscripts “$_m$” and “$_f$” denote mother and  father of the newborn separately. (2)$native$ is a binary variable, 1 for Norwegian nationality, 0 for other nationalities. (3)$img$ is ``immigration background", 1 for person born in Norway to Norwegian parents, 0 for other cases. (4)(Gross) $income$, $wealth$ and $debt$ are in thousand Norwegian kroner (NOK) the year registered.
    \end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/gene.tex <==
\begin{table}[htbp]
\centering
\begin{threeparttable}
\caption{Birth weight and heritable traits \label{tab:gene} }
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
\toprule
 &\multicolumn{4}{c}{\textit{grunnkrets}-(calendar)month FE} &&\multicolumn{4}{c}{postcode-(calendar)month FE} \\
            \cmidrule{2-5} \cmidrule{7-10}   
 &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)} &\multicolumn{1}{c}{(8)}\\
\midrule
\multicolumn{5}{l}{A. Birth weight} \\

$NO$        &      -1.388\sym{**} &      -0.800         &      -1.517\sym{**} &      -0.908              & &        -0.956\sym{**} &      -1.035\sym{*}  &      -0.957\sym{**} &      -1.098\sym{*}   \\
            &     (0.591)         &     (0.866)         &     (0.596)         &     (0.871)              & &       (0.454)         &     (0.575)         &     (0.454)         &     (0.576)          \\
$NO_2$      &       0.119         &      -2.215         &       0.053         &      -2.169              & &        -0.000         &      -1.138         &      -0.265         &      -1.105          \\
            &     (1.696)         &     (2.381)         &     (1.716)         &     (2.396)              & &       (1.141)         &     (1.461)         &     (1.143)         &     (1.460)          \\
$PM_{10}$   &       0.778         &       2.895         &       0.574         &       2.832              & &         1.430         &       2.474         &       1.406         &       2.526\sym{*}   \\
            &     (1.447)         &     (2.238)         &     (1.462)         &     (2.248)              & &       (1.108)         &     (1.503)         &     (1.120)         &     (1.509)          \\
size$_p$    &     no              &         yes         &      no             &             yes          & &        no              &         yes         &      no             &             yes    \\
diabetes  &     no              &         no          &      yes            &             yes          & &        no              &         no          &      yes            &             yes    \\
\midrule
$r^2$       &       0.456         &       0.540         &       0.458         &       0.541              & &         0.318         &       0.406         &       0.319         &       0.407          \\
Obs.        &     241,883         &     118,684         &     239,561         &     118,235              & &       343,605         &     191,150         &     340,946         &     190,553          \\

\midrule
\multicolumn{5}{l}{B. Birth length} \\

$NO$        &      -0.055\sym{*}  &      -0.025         &      -0.054\sym{*}  &      -0.025              & &        -0.021         &      -0.036         &      -0.020         &      -0.038          \\
            &     (0.028)         &     (0.040)         &     (0.029)         &     (0.041)              & &       (0.021)         &     (0.028)         &     (0.021)         &     (0.028)          \\
$NO_2$      &       0.018         &      -0.070         &       0.002         &      -0.072              & &        -0.063         &      -0.062         &      -0.078         &      -0.063          \\
            &     (0.077)         &     (0.108)         &     (0.078)         &     (0.108)              & &       (0.051)         &     (0.066)         &     (0.051)         &     (0.066)          \\
$PM_{10}$   &      -0.034         &       0.120         &      -0.039         &       0.121              & &         0.031         &       0.091         &       0.032         &       0.094          \\
            &     (0.076)         &     (0.103)         &     (0.076)         &     (0.104)              & &       (0.053)         &     (0.071)         &     (0.054)         &     (0.072)          \\
size$_p$    &     no              &         yes         &      no             &             yes          & &        no              &         yes         &      no             &             yes    \\
diabetes  &     no              &         no          &      yes            &             yes          & &        no              &         no          &      yes            &             yes    \\
\midrule
$r^2$       &       0.455         &       0.529         &       0.456         &       0.530              & &         0.318         &       0.398         &       0.319         &       0.399          \\
Obs.        &     228,866         &     112,057         &     226,661         &     111,634              & &       328,366         &     182,348         &     325,784         &     181,787          \\
\bottomrule

\end{tabular}

\begin{tablenotes}
      \small
      \item Notes: (1) Regressions are based on the benchmark model conditional on (calendar) month-\textit{grunnkrets} (column 1-4) or month-postcode (column 5-8) fixed effect, where ``size$_p$'' and ``diabetes'' indicate if parental birth weight/length and diabetes history are controlled for. (2) The independent variables in Panel A and Panel B are birth weight and birth length separately. (3) Cluster robust standard errors at \textit{grunnkrets} level (column 1-4) and postcode level (column 5-8) in parentheses. (4) *** $p < 0.01$, ** $p<0.05$, * $p<0.1$, (5) All pollutants are in $\mu g/m^3$, birth-weight in gram, birth length in millimeter.
    \end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/hetero_inter.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Birth vekt loss -hetero \label{hetero_vekt}}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{vekt}&\multicolumn{1}{c}{vekt}&\multicolumn{1}{c}{vekt}&\multicolumn{1}{c}{vekt}\\
\midrule
$NO$        &      -1.302\sym{**} &      -1.314\sym{**} &      -1.452\sym{**} &      -1.383         \\
            &     (0.609)         &     (0.616)         &     (0.612)         &     (2.044)         \\
\addlinespace
1.boy#c.$NO$&      -0.045         &                     &                     &                     \\
            &     (0.125)         &                     &                     &                     \\
\addlinespace
1.boy    &     121.219\sym{***}&                     &                     &                     \\
            &     (6.192)         &                     &                     &                     \\
\addlinespace
1.$non_{ntv}$#c.$NO$&                     &      -0.261\sym{*}  &                     &                     \\
            &                     &     (0.152)         &                     &                     \\
\addlinespace
1.$non_{ntv}$      &                     &     -53.806\sym{***}&                     &                     \\
            &                     &     (7.377)         &                     &                     \\
\addlinespace
1.$<50th$#c.$NO$&                     &                     &       0.120         &                     \\
            &                     &                     &     (0.143)         &                     \\
\addlinespace
1.$<50th$     &                     &                     &      -6.223         &                     \\
            &                     &                     &     (6.903)         &                     \\
\addlinespace
1.$<25th$#c.$NO$&                     &                     &                     &      -0.415         \\
            &                     &                     &                     &     (0.521)         \\
\addlinespace
1.$<25th$      &                     &                     &                     &     -10.144         \\
            &                     &                     &                     &    (25.162)         \\
\addlinespace
$NO_2$       &      -0.216         &      -0.236         &      -0.106         &       1.450         \\
            &     (1.755)         &     (1.765)         &     (1.709)         &     (5.621)         \\
\addlinespace
$PM_{10}$      &       1.488         &       1.378         &       1.685         &      -0.185         \\
            &     (1.487)         &     (1.490)         &     (1.435)         &     (4.767)         \\
\addlinespace
$age_m$     &      -0.382         &      -0.260         &      -0.369         &      -2.096\sym{**} \\
            &     (0.390)         &     (0.392)         &     (0.392)         &     (1.016)         \\
\addlinespace
$edu_m$        &       8.680\sym{***}&      11.327\sym{***}&      10.145\sym{***}&       8.442\sym{***}\\
            &     (1.352)         &     (1.344)         &     (1.282)         &     (3.249)         \\
\addlinespace
$edu_f$        &       6.703\sym{***}&       7.564\sym{***}&       5.893\sym{***}&       5.037\sym{*}  \\
            &     (1.254)         &     (1.260)         &     (1.214)         &     (2.808)         \\
\midrule
$r^2$       &       0.470         &       0.463         &       0.459         &       0.573         \\
Obs.        &     225,239         &     225,239         &     238,572         &      45,716         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}



\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Birth length loss -hetero \label{hetero_length}}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{length}&\multicolumn{1}{c}{length}&\multicolumn{1}{c}{length}&\multicolumn{1}{c}{length}\\
\midrule
$NO$        &      -0.049\sym{*}  &      -0.053\sym{*}  &      -0.059\sym{**} &      -0.091         \\
            &     (0.029)         &     (0.029)         &     (0.029)         &     (0.094)         \\
\addlinespace
1.boy#c.$NO$&      -0.001         &                     &                     &                     \\
            &     (0.006)         &                     &                     &                     \\
\addlinespace
1.boy    &       7.663\sym{***}&                     &                     &                     \\
            &     (0.283)         &                     &                     &                     \\
\addlinespace
1.$non_{ntv}$#c.$NO$&                     &      -0.001         &                     &                     \\
            &                     &     (0.007)         &                     &                     \\
\addlinespace
1.$non_{ntv}$      &                     &      -2.193\sym{***}&                     &                     \\
            &                     &     (0.337)         &                     &                     \\
\addlinespace
1.$<50th$#c.$NO$&                     &                     &       0.010         &                     \\
            &                     &                     &     (0.007)         &                     \\
\addlinespace
1.$<50th$     &                     &                     &      -0.520         &                     \\
            &                     &                     &     (0.328)         &                     \\
\addlinespace
1.$<25th$#c.$NO$&                     &                     &                     &      -0.019         \\
            &                     &                     &                     &     (0.025)         \\
\addlinespace
1.$<25th$      &                     &                     &                     &      -0.524         \\
            &                     &                     &                     &     (1.218)         \\
\addlinespace
$NO_2$       &      -0.021         &      -0.022         &      -0.009         &       0.108         \\
            &     (0.080)         &     (0.080)         &     (0.077)         &     (0.257)         \\
\addlinespace
$PM_{10}$      &       0.005         &      -0.001         &      -0.001         &      -0.060         \\
            &     (0.076)         &     (0.077)         &     (0.075)         &     (0.223)         \\
\addlinespace
$age_m$     &       0.003         &       0.010         &       0.003         &      -0.057         \\
            &     (0.019)         &     (0.019)         &     (0.019)         &     (0.051)         \\
\addlinespace
$edu_m$        &       0.518\sym{***}&       0.611\sym{***}&       0.570\sym{***}&       0.625\sym{***}\\
            &     (0.064)         &     (0.065)         &     (0.061)         &     (0.160)         \\
\addlinespace
$edu_f$        &       0.293\sym{***}&       0.323\sym{***}&       0.251\sym{***}&       0.225\sym{*}  \\
            &     (0.057)         &     (0.058)         &     (0.055)         &     (0.132)         \\
\midrule
$r^2$       &       0.473         &       0.461         &       0.456         &       0.566         \\
Obs.        &     212,938         &     212,938         &     225,616         &      42,824         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> tables/interp_plt.tex <==
\begin{table}[htbp]
\centering

\begin{threeparttable}

\caption{Ambient air pollutant concentration interpolated in \textit{grunnkrets} with and without $NO$ monitoring stations nearby ($\mu g/m^3$) \label{tab:interp_plt} \vspace{-5pt}}

\begin{tabular}{l*{12}{c}}
\toprule
            &  \multicolumn{5}{c}{with $NO$ stations nearby} & &  \multicolumn{5}{c}{no $NO$ stations nearby}      \\  
            \cmidrule{2-6} \cmidrule{8-12}
 Variable   &     mean&  s.d.& min&max& Obs.& &     mean&  s.d.& min&max& Obs.\\
\midrule
$NO_2$     &    37.14& 11.93& 464&  0& 110  &&    27.95& 16.38 &  5& 55 &  2\\
$O_3$      &    42.89& 12.93& 224&  3&  84  &&    59.00& 11.96 & 21& 94 & 48\\
$PM_{10}$  &    21.23&  6.56& 461&  4& 128  &&    21.89&  8.01 &  0& 59 & 26\\
$PM_{2.5}$ &    10.63&  4.25& 398&  3&  77  &&    10.43&  3.75 &  2& 43 & 13\\
$SO_2$     &     3.22&  4.51& 113&  0&  33  &&    14.20&  8.31 &  0& 54 &  5\\
\bottomrule
\end{tabular}
\begin{tablenotes}
      \small
      \item Notes: (1) Interpolation uses 20 miles as radius and 0.1 as distance power index. (2) Since there are monitoring stations that detect other pollutants, the ``$NO$ omitted'' areas are still urban. (3) Obs. is the number of observations in thousand.
    \end{tablenotes}
\end{threeparttable}

\end{table}


==> tables/meteo.tex <==
\begin{table}[htbp]
\centering
\caption{Meteorological information \label{tab:meteo}}

\begin{tabular}{l*{4}{c}}
\toprule
Meteorology   &        mean&        s.d.&         min&         max\\
\midrule
$temp(\degree{C})$ &       4.93&        7.34&      -32.25&       42.53\\
$humi(\%)$        &       77.25&        9.37&        0.00&      267.57\\
$press(hPa)$       &     988.86&       36.57&     770.14&      1043.76\\
$wind(m/s)$        &       4.33&        2.70&        0.00&       29.30\\
$precip(mm)$      &        3.51&        4.95&       -1.00
\tablefootnote{I kept the negative precipitation values (extremely rare, 2 observation is my working data for benchmark regression) in raw data if the quality code doesn't indicate ``erroneous".
Since the negative values are very close to 0 ($-1mm \sim 0 mm$), I understand it as very dry conditions.}
&      265.00 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/preterm_birth.tex <==
use "rawdata/mfr/mfr_utvidet.dta",clear
keep W18_0160_LOPENR_PERSON UL_TERMIN
rename W18_0160_LOPENR_PERSON lopenr_pers
save "temp/due",replace



cd "/ssb/stamme03/geoh2/xgl"
use "WorkingData/mfr/mfr_luft_20C_wide.dta",clear
replace edum = . if edum == 9
replace eduf = . if eduf == 9

merge 1:1 lopenr_pers using  "temp/due"
keep if _merge == 3
drop _merge

gen ul_year = yofd(UL_TERMIN)
gen ul_mdate = mofd(UL_TERMIN)
gen ul_wdate = wofd(UL_TERMIN)

gen dif_real_ul = wdate - ul_wdate
gen pretm_0 = dif_real_ul < -3
gen pretm_1 = inrange(dif_real_ul,-8,-4)
gen pretm_2 = inrange(dif_real_ul,-14,-9)
gen pretm_3 = inrange(dif_real_ul,-100,-15)




 tab dif_*
dif_real_ul |      Freq.     Percent        Cum.
------------+-----------------------------------
       -261 |          2        0.00        0.00
       -106 |          1        0.00        0.00
        -51 |          1        0.00        0.00
        -46 |          1        0.00        0.00
        -28 |          1        0.00        0.00
        -26 |          3        0.00        0.00
        -25 |          1        0.00        0.00
        -24 |          3        0.00        0.00
        -23 |          5        0.00        0.00
        -22 |          7        0.00        0.00
        -21 |         11        0.00        0.00
        -20 |         14        0.00        0.01
        -19 |         34        0.00        0.01
        -18 |         85        0.01        0.02
        -17 |        265        0.03        0.04
        -16 |        433        0.04        0.09
        -15 |        518        0.05        0.14
        -14 |        672        0.07        0.21
        -13 |        849        0.09        0.30
        -12 |      1,085        0.11        0.41
        -11 |      1,242        0.13        0.53
        -10 |      1,797        0.18        0.72
         -9 |      2,258        0.23        0.95
         -8 |      3,297        0.34        1.28
         -7 |      4,901        0.50        1.78
         -6 |      7,955        0.81        2.60
         -5 |     12,081        1.23        3.83
         -4 |     22,588        2.31        6.14
         -3 |     47,812        4.88       11.02
         -2 |    112,958       11.53       22.55
         -1 |    209,419       21.38       43.92
          0 |    264,755       27.02       70.95
          1 |    202,907       20.71       91.66
          2 |     75,469        7.70       99.36
          3 |      4,603        0.47       99.83
          4 |        297        0.03       99.86
          5 |        103        0.01       99.87
          6 |         25        0.00       99.87
          7 |         14        0.00       99.87
          8 |         14        0.00       99.88
          9 |         13        0.00       99.88
         10 |         17        0.00       99.88
         11 |          5        0.00       99.88
         12 |         13        0.00       99.88
         13 |          8        0.00       99.88
         14 |          7        0.00       99.88
         15 |          5        0.00       99.88
         16 |          5        0.00       99.88
         17 |          4        0.00       99.88
         18 |          9        0.00       99.88
         19 |         22        0.00       99.89
         20 |         36        0.00       99.89
         21 |         43        0.00       99.89
         22 |         63        0.01       99.90
         23 |         44        0.00       99.91
         24 |         18        0.00       99.91
         25 |          9        0.00       99.91
         26 |         12        0.00       99.91
         27 |          5        0.00       99.91
         29 |          2        0.00       99.91
         30 |          1        0.00       99.91
         31 |          2        0.00       99.91
         32 |          3        0.00       99.91
         33 |          1        0.00       99.91
         34 |          4        0.00       99.91
         35 |          4        0.00       99.91
         36 |          6        0.00       99.91
         37 |         14        0.00       99.91
         38 |         12        0.00       99.92
         39 |         22        0.00       99.92
         40 |         19        0.00       99.92
         41 |         23        0.00       99.92
         42 |         19        0.00       99.92
         43 |          8        0.00       99.92
         44 |         14        0.00       99.93
         45 |          6        0.00       99.93
         46 |         20        0.00       99.93
         47 |         23        0.00       99.93
         48 |         40        0.00       99.94
         49 |         60        0.01       99.94
         50 |        119        0.01       99.95
         51 |        167        0.02       99.97
         52 |        152        0.02       99.99
         53 |         90        0.01      100.00
         54 |         25        0.00      100.00
         55 |          4        0.00      100.00
         56 |          1        0.00      100.00
         58 |          1        0.00      100.00
         61 |          1        0.00      100.00
         74 |          1        0.00      100.00
         75 |          1        0.00      100.00
        104 |          1        0.00      100.00
        105 |          3        0.00      100.00
        140 |          1        0.00      100.00
        154 |          1        0.00      100.00
        156 |          1        0.00      100.00
        260 |          1        0.00      100.00
        331 |          1        0.00      100.00
        475 |          1        0.00      100.00
        519 |          1        0.00      100.00
        521 |          3        0.00      100.00
------------+-----------------------------------
      Total |    979,703      100.00



. sum pretm*

    Variable |        Obs        Mean    Std. dev.       Min        Max
-------------+---------------------------------------------------------
     pretm_0 |  1,009,116     .059567    .2366829          0          1
     pretm_1 |  1,009,116    .0503629    .2186927          0          1
     pretm_2 |  1,009,116    .0078316    .0881492          0          1
     pretm_3 |  1,009,116    .0013695    .0369816          0          1














==> tables/se.tex <==
\begin{table}[htbp]
\centering
\caption{Standard error under different assumptions \label{tab:se}}

\begin{threeparttable}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
            &\multicolumn{1}{c}{Birth weight}&\multicolumn{1}{c}{Birth length} \\

\midrule

$NO$         & -0.595\sym{***}& -0.130\sym{*}  \\
$cluster_1$  &(0.141)         &(0.066)   \\
$cluster_2$  &(0.140)         & (0.064)   \\
bootstrap    &(0.145)         & (0.059)  \\
\addlinespace 
$NO_2$       &  0.066         & -0.043 \\
$cluster_1$  &(0.290)         &(0.129)  \\
$cluster_2$  &(0.293)         & (0.132)  \\
bootstrap    &(0.309)         & (0.126)  \\

\addlinespace
$PM_{10}$    &  0.561         &   -0.045 \\
$cluster_1$  &(0.324)         &  (0.141) \\
$cluster_2$  &(0.335)         &  (0.147)  \\
bootstrap    &(0.290)         &   (0.139)  \\

\midrule
$r^2$        &   0.022        &   0.023   \\
Obs.         &   311,283      & 299,982  \\
\bottomrule

\end{tabular}

\begin{tablenotes}
      \subscript
      \item Notes: (1) Standard errors in parentheses, (2) $cluster_1$ means error terms clustered at \textit{grunnkrets} level and  $cluster_2$ at "same mother" level, (3) Significance level is based on bootstrap standard errors, where *** $p < 0.001$, * $p<0.05$, (4) Regression is based on the benchmark regression but only includes \textit{grunnkrets} with more than 100 newborns and the parental nationality is adjusted to a binary variable (1 for Norwegian, 0 for foreigner).
    \end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/spacial_bw.tex <==
\begin{table}[htbp]\centering
\begin{threeparttable}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Spatial endogeneity (birth weight) \label{tab:endo_w}}
\begin{tabular}{l*{6}{c}}
\toprule

            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\midrule

\multicolumn{7}{l}{A. Regression based on column (1) of Table \ref{tab:bm_w}} \\

$NO$        &      -0.407\sym{***}&      -0.602\sym{***}&      -0.623\sym{***}&      -0.209         &      -0.483\sym{***}&      -0.530\sym{***}\\
            &     (0.096)         &     (0.090)         &     (0.086)         &     (0.110)         &     (0.103)         &     (0.098)         \\
\addlinespace
$NO_2$       &       0.136         &       0.116         &       0.048         &      -0.074         &      -0.086         &      -0.141         \\
            &     (0.201)         &     (0.167)         &     (0.156)         &     (0.221)         &     (0.182)         &     (0.173)         \\
Level        &  	 QG          & 		 QP         & 			 QC         &		  MG         & 			 MP         & 		 MC         \\
$r^2$    &    0.023      &    0.019      &    0.006      &    0.023      &    0.019      &    0.007         \\
Obs.        &  463,860         &  463,239         &  463,980         &  463,860         &  463,239         &  463,980         \\


\midrule
\multicolumn{7}{l}{B.Regression based on column (6) of Table \ref{tab:bm_w}} \\

$NO$        &      -0.575\sym{***}&      -0.559\sym{***}&      -0.560\sym{***}&      -0.399\sym{**} &      -0.385\sym{**} &      -0.389\sym{**} \\
            &     (0.123)         &     (0.116)         &     (0.110)         &     (0.139)         &     (0.131)         &     (0.125)         \\
\addlinespace
$NO_2$       &       0.160         &       0.560\sym{*}  &       0.469\sym{*}  &      -0.115         &       0.303         &       0.201         \\
            &     (0.255)         &     (0.219)         &     (0.220)         &     (0.274)         &     (0.241)         &     (0.238)         \\
Level        &        QG           &  QP                 &  QC        		 &        MG            & 		 MP         & 			 MC         \\
$r^2$    &    0.031      &    0.034      &    0.019      &    0.032      &    0.035      &    0.020         \\
Obs.        &  387,426         &  386,757               &  387,504         &  387,426         &  386,757         &  387,504         \\

\bottomrule
\end{tabular}

\begin{tablenotes}
      \small
      \item Notes: (1) Cluster robust standard errors at the level of spatial fixed effect used in regression in parentheses, (2) ***
$p < 0.001$, ** $p<0.01$, * $p<0.05$, (3) Here Q means quarter, M means month, C means municipality,
P means postcode, and G means \textit{grunnkrets}. (4) All pollutants are in $\mu g/m^3$, birth-weight in gram.
    \end{tablenotes}
\end{threeparttable}

\end{table}

==> tables/under.tex <==
\begin{table}[htbp]
\centering
\caption{Underestimation problem using $NO_x$ \label{tab:under}}

\begin{threeparttable}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
            &\multicolumn{1}{c}{weight}&\multicolumn{1}{c}{length}\\
\midrule

\multicolumn{3}{l}{A. $NO_x$ as regressor} \\

$NO_x$       &      -0.251\sym{***}&      -0.059\sym{*} \\
            &     (0.055)          &    (0.025)         \\ 
$PM_{10}$      &       0.414       &       -0.136       \\
            &     (0.286)          &    (0.125)         \\ 
\midrule  
$r^2$       &       0.031          &      0.032         \\ 
Obs.        &  388,008          &    373,611         \\
   
\midrule
\multicolumn{3}{l}{B. Benchmark regression} \\

$NO$        &      -0.575\sym{***}&      -0.114\sym{*} \\ 
            &     (0.123)         &     (0.057)        \\ 
$NO_2$       &       0.160        &       -0.032       \\ 
            &     (0.255)         &     (0.114)        \\ 
$PM_{10}$      &       0.459      &       -0.126       \\ 
            &     (0.286)         &     (0.125)        \\ 
\midrule   
$r^2$       &       0.031         &       0.032        \\ 
Obs.        &  387,426            &  373,034      \\  
\bottomrule
\end{tabular}

\begin{tablenotes}
      \small
      \item Notes: (1)Regression in panel A is also based on the benchmark regression model, (2)Cluster robust s.e. at \textit{grunnkrets} level in parentheses,(3) *** $p < 0.01$, ** $p<0.05$, * $p<0.1$,(4)Pollutants in $\mu g/m^3$, birth-weight in $g$, birth-length in $mm$.
    \end{tablenotes}
\end{threeparttable}
\end{table}
